Trust, but Verify: Evaluating Developer Behavior in Mitigating Security Vulnerabilities in Open-Source Software Projects

This study investigates vulnerabilities in dependencies of sampled open-source software (OSS) projects, the relationship between these and overall project security, and how developers' behaviors and practices influence their mitigation. Through analysis of OSS projects, we have identified common issues in outdated or unmaintained dependencies, including pointer dereferences and array bounds violations, that pose significant security risks. We have also examined developer responses to formal verifier reports, noting a tendency to dismiss potential issues as false positives, which can lead to overlooked vulnerabilities. Our results suggest that reducing the number of direct dependencies and prioritizing well-established libraries with strong security records are effective strategies for enhancing the software security landscape. Notably, four vulnerabilities were fixed as a result of this study, demonstrating the effectiveness of our mitigation strategies.

==> rascunho.tex <==

The C programming language is widely used to develop critical software, such as operating systems, device drivers, and encryption libraries. However, it lacks protection mechanisms, leaving developers in charge of the memory and resource management procedures. Moreover, any lapse in this regard can result in undefined behavior, which exposes a program to security vulnerabilities. It's crucial for developers to be aware of these risks and ensure that pointers used in subtraction operations belong to the same memory segment to prevent these adverse outcomes.

Thereby, software developers now have many multifaceted solutions for program testing using static techniques, which allow users to customize key parameters specific to the desired test scenarios \mbox{\cite{xin2011program, situ2018vanguard, fioraldi2020fuzzing, yamaguchi2013chucky, gui2021uafsan}}.

It is worth mentioning that the complete chain for software verification involves vulnerability identification, vulnerability confirmation, code analysis, and code repair (e.g., patch application and merge requests to a repository). However, that was not possible for all programs mentioned in Section \ref{sec:setup} due to the infrastructure available for each project, the long time necessary for that, or the availability of their respective developers. Anyway, some of the issues found here were reported within the code repositories of VLC, VIM, RUFUS, OpenSSH, CMake, Netdata, Wireshark, OpenSSL, Putty, and Redis, via specific tools or e-mail. In response to the confirmed software vulnerabilities, triggered by fault reports generated by the dedicated tool, remedial patches were subsequently applied. 

According to Xiao {\it et al.} \cite{xiao2014social}, security vulnerabilities are a significant challenge when creating applications with open-source code. Their research investigated several social factors that impact developers' adoption decisions based on a multidisciplinary field of research called \textit{diffusion of innovations}. Its results show that security tools can force developers to build more secure software systems by helping them detect or fix vulnerabilities in source code during implementation phases. In addition, conditions such as concerning behavior and lack of understanding regarding the consequences of security failures were identified in those whose primary activity is code writing. Moreover, while most open-source software projects have large communities contributing to their growth, some are not regularly maintained, which favors security faults.

Jing Zou {\it et al.}~\mbox{\cite{zou2019research}} pointed out a critical perspective: open-source software should be checked according to its supply chain and manufacturer-reserved backdoors. In addition, even when a program does not use specific vulnerable components directly, an element bundled in some linked package (\mbox{\it{e.g.}} third-party library, module, etc.) may cause problems and then affect others by cascading effects defined as transitive dependency. Furthermore, it is essential to examine source code and its documentation to find vulnerabilities. Although many developers are mindful of secure-code best practices, there is no guarantee that they will follow all guidelines during development phases or integrate them into software processes. Moreover, some problems may still exist in the available code as it is challenging to detect security risks before software deployment~\mbox{\cite{gueye2021decade}}.

The issues found and reported in the context of this work were presented based on the counterexample traces provided by LSVerifier. They were also discussed with the respective developers and maintainers, who confirmed some of them and classified others as false positives. Table \mbox{\ref{properties_analysis}} shows the most critical property violations and the corresponding bugs reported via GitHub or e-mail. Although the number of issues informed in the respective repositories may seem low, it is worth mentioning that each of them takes a long time for proper registration, discussion, and correction, which may even span several months. Consequently, we chose the most significant ones for further discussion. 

Regarding CMake, its developers provided a fix for a problem due to a pointer verification before usage in its function $cm\_utf8\_decode\_character$, which caused a pointer dereferencing failure \cite{cmake_issue_1}. Most of its issues are related to third-party libraries. It is crucial for developers to be aware of potential memory management issues so they can take measures to prevent them: for instance, implementing defensive programming practices such as boundary checking on memory access operations. By prioritizing secure memory management practices, developers can help prevent serious security vulnerabilities in their software projects.

The SQLite project's response to this violation reveals another prevalent behavior in the software development community. Developers often dismiss the results from static analyzers, labeling them as ``false positives.'' This perspective stems from the belief that static analyzers frequently produce inaccurate results, leading to unnecessary alarm. The SQLite team's stance is clear: without concrete evidence in the form of an SQL script or specific code that can reproduce an issue, such reports will be disregarded. This approach, while pragmatic, is risky. Relying solely on tangible evidence might overlook potential vulnerabilities that haven't manifested yet but could be exploited in the future. An over-reliance on the historical performance of a codebase, as mentioned by the SQLite team regarding their source tree's ability to confuse static analyzers, can lead to complacency. 

We have also reported another issue caused by a third-party library in OpenSSL \mbox{\cite{openssl_issue_1}}. The developers confirmed that an invalid pointer is dereferenced, which may likely cause a crash in the caller, but they do not consider this to be a vulnerability as many OpenSSL's APIs crash if a null pointer is passed to them. Here, we clearly have a bad practice. Although a problem was found and confirmed, developers often state that a particular condition may never happen as a specific function or method is never invoked the way it should be to provoke it. If an attacker is aware of that and manipulates parameters or even code to create that unfeasible scenario, the problem found here will really happen and may even cause severe loss. Consequently, we also need to encourage a change of behavior, where any problem is handled properly and treated as a priority. Anyway, such a condition should be monitored as it can be a source for an attack resulting in a system crash.

The analysis conducted for Redis revealed multiple violations \cite{redis_issue_1, redis_issue_2}. They included array bound violated (CWE-787), invalid pointer dereference (CWE-476), null pointer dereference (CWE-476), and access to object out-of-bounds (CWE-119). Some were confirmed as false positives \cite{redis_issue_1}. However, a Null pointer was identified in function $completionCallback(ls\rightarrow buf, \&lc)$ without confirming the non-nullity of $ls$ and $ls\rightarrow buf$ \cite{redis_issue_2}. This oversight could lead to the dereferencing of a null pointer. It does pose a risk of undefined behavior if the function is called with a null pointer. Additionally, it should be noted that null checks may be adequate for ensuring pointer validity as a pointer might seem legitimate but can be exploited to reference an invalid memory address. This nuance highlights the importance of comprehensive pointer validation prior to usage. The developers dismissed this potential issue by claiming that a function or method will never be called in a certain way that triggers a problem, despite confirmation of the issue. This is considered a bad practice.

It's essential to recognize that while static analyzers might produce false positives, they can also pinpoint genuine issues that might be overlooked during manual code reviews. It is crucial for developers to strike a balance. While it's unreasonable to expect teams to act on every single report from a static analyzer, completely ignoring them isn't the solution either. A more collaborative approach, where the reporter and the development team work together to validate and address potential issues, can lead to more secure and robust software. After all, the ultimate goal should be to ensure the software's integrity and safeguard it from potential threats, regardless of their origin.

In summary, as seen in counterexample logs and bug reports validation, third-party libraries seem to be the biggest problem. Functions from other libraries that are called in software modules should always be carefully checked by developers as they can be dangerous. Moreover, given that C programs often use pointers to access arrays and those are usually passed as arguments to functions, such a condition can bring serious security issues.

-----------------

Title:
Evaluating Developer Behavior in Mitigating Security Vulnerabilities in Open-Source C Projects

% https://www.computer.org/csdl/journal/tq/5555/01/10400834/1TKMJQ7fo7S

Introduction
The C programming language is widely used to develop critical software, such as operating systems, device drivers, and encryption libraries. However, it lacks protection mechanisms, leaving developers in charge of memory and resource management. Any lapse in this regard can result in undefined behavior, exposing a program to security vulnerabilities. It's crucial for developers to be aware of these risks and ensure that pointers used in subtraction operations belong to the same memory segment to prevent these adverse outcomes.

According to Xiao et al. \cite{xiao2014social}, security vulnerabilities are a significant challenge when creating applications with open-source code. Their research investigated several social factors impacting developers' adoption decisions based on a multidisciplinary field of research called diffusion of innovations. The results show that security tools can force developers to build more secure software systems by helping them detect or fix vulnerabilities in the source code during implementation phases. In addition, conditions such as concerning behavior and lack of understanding regarding the consequences of security failures were identified in those whose primary activity is code writing. While most open-source software projects have large communities contributing to their growth, some are not regularly maintained, which favors security faults.

Jing Zou et al. \cite{zou2019research} pointed out a critical perspective: open-source software should be checked according to its supply chain and manufacturer-reserved backdoors. Even when a program does not use specific vulnerable components directly, an element bundled in some linked package (e.g., third-party library, module, etc.) may cause problems and affect others by cascading effects defined as transitive dependency. It is essential to examine the source code and its documentation to find vulnerabilities. Although many developers are mindful of secure-code best practices, there is no guarantee that they will follow all guidelines during development phases or integrate them into software processes. Moreover, some problems may still exist in the available code as it is challenging to detect security risks before software deployment \cite{gueye2021decade}.

Methodology
Software developers now have many multifaceted solutions for program testing using static techniques, which allow users to customize key parameters specific to the desired test scenarios \cite{xin2011program, situ2018vanguard, fioraldi2020fuzzing, yamaguchi2013chucky, gui2021uafsan}. The complete chain for software verification involves vulnerability identification, vulnerability confirmation, code analysis, and code repair (e.g., patch application and merge requests to a repository). However, this was not possible for all programs mentioned in Section \ref{sec
} due to the infrastructure available for each project, the time required, or the availability of their respective developers.

The issues found and reported in the context of this work were based on the counterexample traces provided by LSVerifier. They were also discussed with the respective developers and maintainers, who confirmed some of them and classified others as false positives.

Results
Some of the issues found were reported within the code repositories of VLC, VIM, RUFUS, OpenSSH, CMake, Netdata, Wireshark, OpenSSL, Putty, and Redis via specific tools or email. In response to the confirmed software vulnerabilities triggered by fault reports generated by the dedicated tool, remedial patches were subsequently applied.

Regarding CMake, its developers provided a fix for a problem due to a pointer verification before usage in its function $cm_utf8_decode_character$, which caused a pointer dereferencing failure \cite{cmake_issue_1}. Most of its issues are related to third-party libraries. It is crucial for developers to be aware of potential memory management issues so they can take measures to prevent them. For instance, implementing defensive programming practices such as boundary checking on memory access operations. By prioritizing secure memory management practices, developers can help prevent serious security vulnerabilities in their software projects.

The SQLite project's response to this violation reveals another prevalent behavior in the software development community. Developers often dismiss the results from static analyzers, labeling them as "false positives." This perspective stems from the belief that static analyzers frequently produce inaccurate results, leading to unnecessary alarm. The SQLite team's stance is clear: without concrete evidence in the form of an SQL script or specific code that can reproduce an issue, such reports will be disregarded. This approach, while pragmatic, is risky. Relying solely on tangible evidence might overlook potential vulnerabilities that haven't manifested yet but could be exploited in the future. An over-reliance on the historical performance of a codebase, as mentioned by the SQLite team regarding their source tree's ability to confuse static analyzers, can lead to complacency.

We also reported another issue caused by a third-party library in OpenSSL \cite{openssl_issue_1}. The developers confirmed that an invalid pointer is dereferenced, which may likely cause a crash in the caller, but they do not consider this to be a vulnerability as many OpenSSL APIs crash if a null pointer is passed to them. Here, we clearly have a bad practice. Although a problem was found and confirmed, developers often state that a particular condition may never happen as a specific function or method is never invoked in the way it should be to provoke it. If an attacker is aware of that and manipulates parameters or even code to create that unfeasible scenario, the problem found here will really happen and may even cause severe loss. Consequently, we also need to encourage a change of behavior, where any problem is handled properly and treated as a priority. Such a condition should be monitored as it can be a source for an attack resulting in a system crash.

The analysis conducted for Redis revealed multiple violations \cite{redis_issue_1, redis_issue_2}. They included array bound violation (CWE-787), invalid pointer dereference (CWE-476), null pointer dereference (CWE-476), and access to object out-of-bounds (CWE-119). Some were confirmed as false positives \cite{redis_issue_1}. However, a null pointer was identified in function $completionCallback(ls\rightarrow buf, &lc)$ without confirming the non-nullity of $ls$ and $ls\rightarrow buf$ \cite{redis_issue_2}. This oversight could lead to the dereferencing of a null pointer, posing a risk of undefined behavior if the function is called with a null pointer. Additionally, null checks may be inadequate for ensuring pointer validity as a pointer might seem legitimate but can be exploited to reference an invalid memory address. This nuance highlights the importance of comprehensive pointer validation prior to usage. The developers dismissed this potential issue by claiming that a function or method will never be called in a certain way that triggers a problem, despite confirmation of the issue. This is considered a bad practice.

Conclusion
While static analyzers might produce false positives, they can also pinpoint genuine issues that might be overlooked during manual code reviews. It is crucial for developers to strike a balance. While it is unreasonable to expect teams to act on every single report from a static analyzer, completely ignoring them isn't the solution either. A more collaborative approach, where the reporter and the development team work together to validate and address potential issues, can lead to more secure and robust software. The ultimate goal should be to ensure the software's integrity and safeguard it from potential threats, regardless of their origin.

In summary, as seen in counterexample logs and bug reports validation, third-party libraries seem to be the biggest problem. Functions from other libraries that are called in software modules should always be carefully checked by developers as they can be dangerous. Given that C programs often use pointers to access arrays and these are usually passed as arguments to functions, such a condition can bring serious security issues.
